Shot noise-mitigated secondary electron imaging with ion count-aided microscopy

Modern science is dependent on imaging on the nanoscale, often achieved through processes that detect secondary electrons created by a highly focused incident charged particle beam. Multiple types of measurement noise limit the ultimate trade-off between the image quality and the incident particle dose, which can preclude useful imaging of dose-sensitive samples. Existing methods to improve image quality do not fundamentally mitigate the noise sources. Furthermore, barriers to assigning a physically meaningful scale make the images qualitative. Here we introduce ion count-aided microscopy (ICAM), which is a quantitative imaging technique that uses statistically principled estimation of the secondary electron yield. With a readily implemented change in data collection, ICAM substantially reduces source shot noise. In helium ion microscopy, we demonstrate 3x dose reduction and a good match between these empirical results and theoretical performance predictions. ICAM facilitates imaging of fragile samples and may make imaging with heavier particles more attractive.

==> textMacros.tex <==
%---------- Abbreviations -----------------------------------------------------
\def\dB{~\mathrm{dB}}

%---------- Typesetting mathematics --------------------------------------------
\newcommand{\0}{{\mathbf 0}}
\newcommand{\1}{{\mathbf 1}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\U}{\ensuremath{\mathbb{U}}}
\newcommand{\Error}{\ensuremath{\mathcal{E}}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\J}{\ensuremath{\mathcal{J}}}
\newcommand{\K}{\ensuremath{\mathcal{K}}}
\newcommand{\Pcal}{\ensuremath{\mathcal{P}}}

\newcommand{\Rn}{\ensuremath{\mathbb{R}^{\dimn}}}
\newcommand{\Rm}{\ensuremath{\mathbb{R}^{\dimm}}}
\newcommand{\Rtwo}{\ensuremath{\mathbb{R}^2}}
\newcommand{\Rthree}{\ensuremath{\mathbb{R}^3}}
\newcommand{\Cn}{\ensuremath{\mathbb{C}^{\dimn}}}
\newcommand{\Cm}{\ensuremath{\mathbb{C}^{\dimm}}}
\newcommand{\Ctwo}{\ensuremath{\mathbb{C}^2}}
\newcommand{\Qn}{\ensuremath{\mathbb{Q}^{\dimn}}}
\newcommand{\CZ}{\ensuremath{\mathbb{C}^{\Z}}}
\newcommand{\CR}{\ensuremath{\mathbb{C}^{\R}}}
\newcommand{\Cab}{\ensuremath{\mathbb{C}^{[a,b]}}}

\newcommand{\lZN}{\ensuremath{\ell(\mathbb{Z}_{\dimn})}}
\newcommand{\lone}{\ensuremath{\ell^1}}
\newcommand{\ltwo}{\ensuremath{\ell^2}}
\newcommand{\lp}{\ensuremath{\ell^p}}
\newcommand{\linfty}{\ensuremath{\ell^\infty}}
\newcommand{\lpZ}{\ensuremath{\ell^p(\mathbb{Z})}}
\newcommand{\lqZ}{\ensuremath{\ell^q(\mathbb{Z})}}
\newcommand{\lzero}{\ensuremath{\ell^0}}
\newcommand{\lzeroZ}{\ensuremath{\ell^0(\mathbb{Z})}}
\newcommand{\loneZ}{\ensuremath{\ell^1(\mathbb{Z})}}
\newcommand{\ltwoZ}{\ensuremath{\ell^2(\mathbb{Z})}}
\newcommand{\ltwoK}{\ensuremath{\ell^2(\K)}}
%\newcommand{\ltwok}{\ensuremath{\ell^2(\{-(k_s-1)/2,\, \ldots,\, (k_s-1)/2\})}}
\newcommand{\ltwok}{\ensuremath{\ell^2(\{-\half(k_s-1),\, \ldots,\, \half(k_s-1)\})}}
\newcommand{\linftyZ}{\ensuremath{\ell^\infty(\mathbb{Z})}}
\newcommand{\loneZtwo}{\ensuremath{\ell^1(\mathbb{Z}^2)}}
\newcommand{\ltwoZtwo}{\ensuremath{\ell^2(\mathbb{Z}^2)}}
\newcommand{\linftyZtwo}{\ensuremath{\ell^\infty(\mathbb{Z}^2)}}
\newcommand{\Lone}{\ensuremath{\mathcal{L}^1}}
\newcommand{\Ltwo}{\ensuremath{\mathcal{L}^2}}
\newcommand{\Lp}{\ensuremath{\mathcal{L}^p}}
\newcommand{\LpR}{\ensuremath{\mathcal{L}^p(\mathbb{R})}}
\newcommand{\Lpab}{\ensuremath{\mathcal{L}^p([a,\, b])}}
\newcommand{\LtwoR}{\ensuremath{\mathcal{L}^2(\mathbb{R})}}
\newcommand{\Ltwoab}{\ensuremath{\mathcal{L}^2([a,\, b])}}
%\newcommand{\LoneT}{\ensuremath{\mathcal{L}^1([-T/2,T/2))}}
%\newcommand{\LtwoT}{\ensuremath{\mathcal{L}^2([-T/2,T/2))}}
\newcommand{\LoneT}{\ensuremath{\mathcal{L}^1([-\half T,\, \half T))}}
\newcommand{\LtwoT}{\ensuremath{\mathcal{L}^2([-\half T,\, \half T))}}
\newcommand{\LtwoMpipi}{\ensuremath{\mathcal{L}^2([-\pi,\,\pi))}}
\newcommand{\LtwoZeroOne}{\ensuremath{\mathcal{L}^2([0,\,1))}}
\newcommand{\LoneR}{\ensuremath{\mathcal{L}^1(\mathbb{R})}}
\newcommand{\LinftyR}{\ensuremath{\mathcal{L}^{\infty}(\mathbb{R})}}
\newcommand{\LtwoRtwo}{\ensuremath{\mathcal{L}^2(\mathbb{R}^2)}}
\newcommand{\Linfty}{\ensuremath{\mathcal{L}^\infty}}
\newcommand{\loneN}{\ensuremath{\ell^1(\mathbb{N})}}
\newcommand{\ltwoN}{\ensuremath{\ell^2(\mathbb{N})}}
\newcommand{\linftyN}{\ensuremath{\ell^\infty(\mathbb{N})}}

\newcommand{\Rlone}{\ensuremath{\R\ell^1}}
\newcommand{\Rltwo}{\ensuremath{\R\ell^2}}
\newcommand{\Rlp}{\ensuremath{\R\ell^p}}
\newcommand{\Rlinfty}{\ensuremath{\R\ell^\infty}}
\newcommand{\RlpZ}{\ensuremath{\R\ell^p(\mathbb{Z})}}
\newcommand{\RlzeroZ}{\ensuremath{\R\ell^0(\mathbb{Z})}}
\newcommand{\RloneZ}{\ensuremath{\R\ell^1(\mathbb{Z})}}
\newcommand{\RltwoZ}{\ensuremath{\R\ell^2(\mathbb{Z})}}
\newcommand{\RlinftyZ}{\ensuremath{\R\ell^\infty(\mathbb{Z})}}
\newcommand{\RloneZtwo}{\ensuremath{\R\ell^1(\mathbb{Z}^2)}}
\newcommand{\RltwoZtwo}{\ensuremath{\R\ell^2(\mathbb{Z}^2)}}
\newcommand{\RlinftyZtwo}{\ensuremath{\R\ell^\infty(\mathbb{Z}^2)}}
\newcommand{\RLone}{\ensuremath{\R\mathcal{L}^1}}
\newcommand{\RLtwo}{\ensuremath{\R\mathcal{L}^2}}
\newcommand{\RLp}{\ensuremath{\R\mathcal{L}^p}}
\newcommand{\RLpR}{\ensuremath{\R\mathcal{L}^p(\mathbb{R})}}
\newcommand{\RLtwoR}{\ensuremath{\R\mathcal{L}^2(\mathbb{R})}}
\newcommand{\RLoneR}{\ensuremath{\R\mathcal{L}^1(\mathbb{R})}}
\newcommand{\RLinftyR}{\ensuremath{\R\mathcal{L}^{\infty}(\mathbb{R})}}
\newcommand{\RLtwoPmone}{\ensuremath{\R\mathcal{L}^2([-1,\,1])}}
\newcommand{\RLtwoab}{\ensuremath{\R\mathcal{L}^2([a,\,b])}}
\newcommand{\RLtwoRtwo}{\ensuremath{\R\mathcal{L}^2(\mathbb{R}^2)}}
\newcommand{\RLinfty}{\ensuremath{\R\mathcal{L}^\infty}}

\newcommand{\poly}[2]{\mathcal{P}_{#1}{#2}} % polynomial spaces
\def\Leg{{\bar{L}}}  % normalized Legendre polynomial
\def\Lag{{\ell}}     % Lagrange polynomial
\newcommand{\polyLS}[1]{p_{#1}^{\rm{LS}}}  % not currently used

\newcommand{\cd}{\ensuremath{\mathcal{\kappa}}}
%\def\S{{S}} % range of interpolation operator
%\def\Sperp{{S^\perp}}
%\def\Stilde{{\widetilde{S}}}
                      % orthogonal complement of null space of sampling operator
%\def\Stildeperp{{\widetilde{S}^\perp}}
\def\Ydet{{Y_{\rm det}}}
\def\Yhigh{{Y_{\rm high}}}
\def\Ylow{{Y_{\rm low}}}
\newcommand{\PRestrict}[1]{1_{#1}}
\def\T{{\top}}

\newcommand{\ip}[2]{\langle #1, \, #2 \rangle}
\newcommand{\iplarge}[2]{\left\langle #1, \, #2 \right\rangle}
\newcommand{\ipsmall}[2]{\langle #1, \, #2 \rangle}
\newcommand{\lrip}[2]{\left\langle #1, \, #2 \right\rangle}
\newcommand{\bigip}[2]{\bigl\langle #1, \, #2 \bigr\rangle}
\newcommand{\Bigip}[2]{\Bigl\langle #1, \, #2 \Bigr\rangle}
\newcommand{\biggip}[2]{\biggl\langle #1, \, #2 \biggr\rangle}
\newcommand{\Biggip}[2]{\Biggl\langle #1, \, #2 \Biggr\rangle}
\newcommand{\ipk}[2]{\langle #1, \, #2 \rangle_{k}}
%\newcommand{\ipklarge}[2]{\left\langle #1, \, #2 \right\rangle_{k}}
\newcommand{\ipksmall}[2]{\langle #1, \, #2 \rangle_{k}}
\newcommand{\ipn}[2]{\langle #1, \, #2 \rangle_{n}}
%\newcommand{\ipnlarge}[2]{\left\langle #1, \, #2 \right\rangle_{n}}
\newcommand{\ipnsmall}[2]{\langle #1, \, #2 \rangle_{n}}
\newcommand{\bigipn}[2]{\bigl\langle #1, \, #2 \bigr\rangle_{n}}
\newcommand{\Bigipn}[2]{\Bigl\langle #1, \, #2 \Bigr\rangle_{n}}
%\newcommand{\biggipn}[2]{\biggl\langle #1, \, #2 \biggr\rangle_{n}}
\newcommand{\biggipn}[2]{\biggl\langle #1, \, #2 \biggr\rangle{\bigg.\!}_n}
%\newcommand{\Biggipn}[2]{\Biggl\langle #1, \, #2 \Biggr\rangle_{n}}
\newcommand{\Biggipn}[2]{\Biggl\langle #1, \, #2 \Biggr\rangle{\Bigg.\!}_n}
\newcommand{\ipt}[2]{\langle #1, \, #2 \rangle_{t}}
%\newcommand{\iptlarge}[2]{\left\langle #1, \, #2 \right\rangle_{t}}
\newcommand{\iptsmall}[2]{\langle #1, \, #2 \rangle_{t}}
\newcommand{\bigipt}[2]{\bigl\langle #1, \, #2 \bigr\rangle_{t}}
%\newcommand{\Bigipt}[2]{\Bigl\langle #1, \, #2 \Bigr\rangle_{t}}
\newcommand{\Bigipt}[2]{\Bigl\langle #1, \, #2 \Bigr\rangle{\Big.\!}_t}
%\newcommand{\biggipt}[2]{\biggl\langle #1, \, #2 \biggr\rangle_{t}}
\newcommand{\biggipt}[2]{\biggl\langle #1, \, #2 \biggr\rangle{\bigg.\!}_t}
%\newcommand{\Biggipt}[2]{\Biggl\langle #1, \, #2 \Biggr\rangle_{t}}
\newcommand{\Biggipt}[2]{\Biggl\langle #1, \, #2 \Biggr\rangle{\Bigg.\!}_t}
% Think "X" for "eXplicit"
\newcommand{\ipX}[3]{\langle #1, \, #2 \rangle_{#3}}
%\newcommand{\ipXlarge}[3]{\left\langle #1, \, #2 \right\rangle_{#3}}
\newcommand{\ipXsmall}[3]{\langle #1, \, #2 \rangle_{#3}}

\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\lrabs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\bigabs}[1]{\bigl\lvert #1 \bigr\rvert}
\newcommand{\Bigabs}[1]{\Bigl\lvert #1 \Bigr\rvert}
\newcommand{\biggabs}[1]{\biggl\lvert #1 \biggr\rvert}
\newcommand{\Biggabs}[1]{\Biggl\lvert #1 \Biggr\rvert}
\newcommand{\norm}[1]{\lVert #1 \rVert}
\newcommand{\lrnorm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\bignorm}[1]{\bigl\lVert #1 \bigr\rVert}
\newcommand{\Bignorm}[1]{\Bigl\lVert #1 \Bigr\rVert}
\newcommand{\biggnorm}[1]{\biggl\lVert #1 \biggr\rVert}
\newcommand{\Biggnorm}[1]{\Biggl\lVert #1 \Biggr\rVert}
\newcommand{\conv}[2]{#1 \ast #2}
\newcommand{\convX}[3]{#1 \ast_{#3} #2}
\newcommand{\convXsmall}[3]{#1 \ast_{#3} #2}
\newcommand{\convXlarge}[3]{\left( #1 \ast #2 \right)_{#3}}
\newcommand{\convn}[2]{#1 \ast_{n} #2}
\newcommand{\convt}[2]{#1 \ast_{t} #2}
\newcommand{\circConv}[2]{#1 \circledast #2}
\newcommand{\circConvX}[3]{#1 \circledast_{#3} #2}

\newcommand{\zt}{\ensuremath{z}-transform}
\newcommand{\zT}{\ensuremath{z}-Transform}

\newcommand{\twovector}[2]{\begin{bmatrix} #1 \\ #2 \end{bmatrix}}
\newcommand{\twovectorXtra}[2]{\begin{bmatrix} #1 \\[\matrixSkip] #2 \end{bmatrix}}
\newcommand{\threevector}[3]{\begin{bmatrix} #1 \\ #2 \\ #3 \end{bmatrix}}
\newcommand{\tworow}[2]{\begin{bmatrix} #1 & #2 \end{bmatrix}}
\newcommand{\twobytwo}[4]{\begin{bmatrix} #1 & #2 \\ #3 & #4 \end{bmatrix}}
\newcommand{\twobytworr}[4]{\begin{bmatrix} #1 & #2 \\ #3 & #4 \end{bmatrix}}
\newcommand{\parentwobytwo}[4]{\left(\begin{bmatrix} #1 & #2 \\ #3 & #4 \end{bmatrix}\right)}
\newcommand{\twobythree}[6]{\begin{bmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \end{bmatrix}}
\newcommand{\threebythree}[9]{\begin{bmatrix} #1 & #2 & #3 \\ #4 & #5 & #6 \\ #7 & #8 & #9 \end{bmatrix}}

\newcommand{\setphi}{\ensuremath{\Phi = \{\varphi_i\}_{i \in \I}}}
\newcommand{\setphitilde}{\ensuremath{\widetilde{\Phi} = \{\widetilde{\varphi_i}\}_{i \in \I}}}
\newcommand{\setphim}{\ensuremath{\Phi = \{\varphi_i\}_{i=1}^{\dimm}}}
\newcommand{\uhat}{\widehat{u}}
\newcommand{\yhat}{\widehat{y}}
\newcommand{\xhat}{\widehat{x}}
\newcommand{\That}{\widehat{T}}
\newcommand{\Xhat}{\widehat{X}}
\newcommand{\Zhat}{\widehat{Z}}
\newcommand{\XhatMMSE}{\widehat{\mathrm{x}}_{\rm MMSE}}
\newcommand{\XhatMAP}{\widehat{\mathrm{x}}_{\rm MAP}}
\newcommand{\XhatML}{\widehat{\mathrm{x}}_{\rm ML}}
\newcommand{\xhatL}[1]{\widehat{x}_{#1}}
\newcommand{\yhatL}[1]{\widehat{y}_{#1}}
\def\SNR{\mbox{\small \sffamily SNR}}
\newcommand{\xhatLin}{\widehat{x}_{\rm L}}
%--
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}
\newcommand{\xhatNL}[1]{\widecheck{x}_{#1}}
\newcommand{\yhatNL}[1]{\widecheck{y}_{#1}}
\newcommand{\zhatNL}[1]{\widecheck{z}_{#1}}
\def\xcheck{\widecheck{x}}
%--
\newcommand{\eL}{e_{\rm L}}
\newcommand{\eNL}{e_{\rm NL}}
\newcommand{\epsL}{\varepsilon_{\rm L}}
\newcommand{\epsNL}{\varepsilon_{\rm NL}}
\newcommand{\Ghat}{\widehat{G}}
\newcommand{\Yhat}{\widehat{Y}}
\newcommand{\alphaHat}{\widehat{\alpha}}
\newcommand{\pinv}[1]{{#1}^{\dagger}}  % pseudoinverse
\newcommand{\ahat}{\widehat{\alpha}}
\newcommand{\ghat}{\widehat{g}}

% Complexity
\newcommand{\Ca}{\ensuremath{\nu}}
\newcommand{\Cmu}{\ensuremath{\mu}}

\newcommand{\Frac}[2]{{{#1}/{#2}}}  % an "inert" form of \frac
\newcommand{\pFrac}[2]{{({#1}/{#2})}}  % an "inert" form of \frac
\newcommand{\bigFrac}[2]{{{#1}{\big /}{#2}}}  % an "inert" form of \frac
\newcommand{\BigFrac}[2]{{{#1}{\Big /}{#2}}}  % an "inert" form of \frac
\newcommand{\tsfrac}[2]{{\textstyle \frac{#1}{#2}}}
%\newcommand{\zt}{\ensuremath{z}-transform}
%\newcommand{\DFT}{\operatorname{DFT}}
\newcommand{\bias}{\operatorname{bias}}
\newcommand{\MSE}{\operatorname{MSE}}
\newcommand{\MSEconv}{\operatorname{MSE}_{\rm conv}}
\newcommand{\MSEICA}{\operatorname{MSE}_{\rm ICA}}
\newcommand{\REconv}{\operatorname{RE}_{\rm conv}}
\newcommand{\REICA}{\operatorname{RE}_{\rm ICA}}
\newcommand{\LFT}{\operatorname{LFT}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\lcm}{\operatorname{lcm}}

\newcommand{\ds}{\displaystyle}
\newcommand{\ts}{\textstyle}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\eeqan}{\end{eqnarray*}}
\newcommand{\nn}{\nonumber}

\newcommand{\eqlabel}[1]{ \stackrel{(#1)}{=} }
\newcommand{\glabel}[1]{ \stackrel{(#1)}{>} }
\newcommand{\llabel}[1]{ \stackrel{(#1)}{<} }
\newcommand{\geqlabel}[1]{ \stackrel{(#1)}{\geq} }
\newcommand{\leqlabel}[1]{ \stackrel{(#1)}{\leq} }
\newcommand{\approxlabel}[1]{ \stackrel{(#1)}{\approx} }
\newcommand{\ralabel}[1]{ \stackrel{(#1)}{\rightarrow} }
\newcommand{\simlabel}[1]{ \stackrel{(#1)}{\sim} }
\newcommand{\inlabel}[1]{ \stackrel{(#1)}{\in} }

% Equations with cases
\newcommand{\openCase}  {\left\{ \begin{array}{@{\,}ll}}
\newcommand{\openCasell}{\left\{ \begin{array}{@{\,}ll}}
\newcommand{\openCasecl}{\left\{ \begin{array}{@{\,}cl}}
\newcommand{\openCaserl}{\left\{ \begin{array}{@{\,}rl}}
\newcommand{\openCaseTablell}{\left\{ \begin{array}{@{}ll}}
\newcommand{\openCaseTablecl}{\left\{ \begin{array}{@{}cl}}
\newcommand{\openCaseTablerl}{\left\{ \begin{array}{@{}rl}}
\newcommand{\closeCase} {\end{array} \right.}

\def\doubleline{\addtolength{\baselineskip}{12pt}}
\def\suminf#1{\sum_{#1=-\infty}^{\infty}}
\def\sumfin{\sum_{i=1}^{n}}
\def\intinf{\int_{-\infty}^{\infty}}
\def\intMpipi{\int_{-\pi}^{\pi}}
\def\intT{\int_{-T/2}^{T/2}}
\def\intTeps{\int_{-\epsilon}^{T-\epsilon}}
\def\w{\omega}
\def\jw{j\omega}
\def\ejw{e^{j\omega}}
\def\emjw{e^{-j\omega}}
\def\ejwt{e^{j\omega t}}
\def\emjwt{e^{-j\omega t}}
\def\ejtpTkt{e^{j (2 \pi/T) k t}}
\def\emjtpTkt{e^{-j (2 \pi/T) k t}}
\def\ejwn{e^{j\omega n}}
\def\ejwk{e^{j\omega k}}
\def\emjwn{e^{-j\omega k}}
\def\emjwk{e^{-j\omega k}}
\def\dw{d\omega}
\def\Half{{\frac{1}{2}}}
\def\half{{\textstyle\frac{1}{2}}}
\def\halfpi{\half\pi}
\def\halfT{\half T}
\def\halftnot{\half t_0}
\def\halfwnot{\half\w_0}
\def\Halfwnot{\Half\w_0}
\def\iHalf{{\Frac{1}{2}}}        % Inert version of \Half
\def\Third{{\frac{1}{3}}}
\def\third{{\textstyle\frac{1}{3}}}
\def\iThird{{\Frac{1}{3}}}        % Inert version of \Half
\def\Oosrt{{\frac{1}{\sqrt{2}}}} % Read as "one over square-root two"
\def\iOosrt{{\Frac{1}{\sqrt{2}}}} % Inert version of \Oosrt
\def\oosrt{{\textstyle\frac{1}{\sqrt{2}}}}
\def\OosrN{{\frac{1}{\sqrt{N}}}} % Read as "one over square-root N"
\def\iOosrN{{\Frac{1}{\sqrt{N}}}} % Inert version of \OosrN
\def\oosrN{{\textstyle\frac{1}{\sqrt{N}}}}
\def\OosrT{{\frac{1}{\sqrt{T}}}} % Read as "one over square-root T"
\def\iOosrT{{\Frac{1}{\sqrt{T}}}} % Inert version of \OosrT
\def\oosrT{{\textstyle\frac{1}{\sqrt{T}}}}
\def\oosrTs{{\textstyle\frac{1}{\sqrt{T_s}}}}
\def\twopiT{{\frac{2\pi}{T}}}
% \def\tstwopiT{{\textstyle\frac{2\pi}{T}}}
\def\tstwopiT{{\frac{2\pi}{T}}}
\def\tsminus{{\textstyle-}}
\def\kToInfty{\stackrel{k \to \infty}{\longrightarrow}}

\def\PhiTilde{\widetilde{\Phi}}
\def\phiTilde{\widetilde{\varphi}}
\def\PsiTilde{\widetilde{\Psi}}
\def\psiTilde{\widetilde{\psi}}
\def\gtilde{\widetilde{g}}
\def\gtildes{\widetilde{g}^*}
\def\htilde{\widetilde{h}}
\def\Ntilde{\widetilde{\dimn}}
\def\Gtilde{\widetilde{G}}
\def\Htilde{\widetilde{H}}
\def\Ltilde{\widetilde{L}}
\def\mtilde{\widetilde{m}}
\def\Mtilde{\widetilde{M}}
\def\stilde{\widetilde{s}}
\def\ttilde{\widetilde{t}}
\def\Ttilde{\widetilde{T}}
\def\Utilde{\widetilde{U}}
\def\wtilde{\widetilde{\w}}
\def\xtilde{\widetilde{x}}
\def\Xtilde{\widetilde{X}}
\def\ytilde{\widetilde{y}}
\def\Ytilde{\widetilde{Y}}
\def\Ztilde{\widetilde{Z}}
\def\alphatilde{\widetilde{\alpha}}
\def\betatilde{\widetilde{\beta}}
\def\PTilde{\widetilde{P}}
\def\lmin{\lambda_{\rm min}}
\def\lmax{\lambda_{\rm max}}
\def\lminTilde{\widetilde{\lambda}_{\rm min}}
\def\lmaxTilde{\widetilde{\lambda}_{\rm max}}
\def\smin{\sigma_{\rm min}}
\def\smax{\sigma_{\rm max}}
\def\xmin{x_{\rm min}}
\def\xmax{x_{\rm max}}
\def\wmax{\w_{\rm max}}

\def\btilde{\widetilde{\beta}}

\newcommand{\BL}[1]{{\mathrm{BL}}[-#1,\,#1]}  % Subspace of bandlimited functions/sequences
\newcommand{\BLk}[1]{{\mathrm{BL}}\{-#1,\,\ldots,\,#1\}}  % Subspace of bandlimited functions/sequences
\newcommand{\xBL}{x_{\rm BL}}
%\newcommand{\spline}[2]{S(#1;#2)}
\newcommand{\spline}[2]{S_{#1,#2}}
\newcommand{\Bs}[1]{\beta^{(#1)}}
\newcommand{\BsFT}[1]{B^{(#1)}}
\newcommand{\Bstilde}[1]{\betatilde^{(#1)}}
\newcommand{\Bsperp}[1]{\beta_\perp^{(#1)}}
\newcommand{\Bsplus}[1]{\beta_+^{(#1)}}
\newcommand{\BsplusFT}[1]{B_+^{(#1)}}
\newcommand{\Bsplustilde}[1]{\betatilde_+^{(#1)}}
\newcommand{\Bsdiff}[1]{\Delta^{(#1)}}
\newcommand{\Bsint}[1]{\zeta^{(#1)}}
\newcommand{\Ba}[1]{h^{(#1)}}
\newcommand{\BA}[1]{H^{(#1)}}

\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\adj}{adj}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\round}{round}
\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\Support}{support}
\def\CSpan{\mathop{\overline{\mathrm{span}}}}
\def\range{\mathcal{R}}
\def\ker{\mathcal{N}}
\def\polyphase{\mathcal{P}} % How is this used? (VKG 29 Jul 2012)
\def\roc{\mathrm{ROC}}
%\renewcommand{\P}[1]{\textbf{P}\left({#1}\right)} % Probability
\renewcommand{\P}[1]{\mathrm{P}\left({#1}\right)} % Probability
\newcommand{\iP}[1]{\mathrm{P}({#1})} % Probability (inline)
\def\smid{\,|\,}  % Like \mid, but with less space; use for conditioning
\def\sMid{\,;\,}  % Version of \smid for non-Bayesian case
%\newcommand{\E}[1]{\textbf{E}\left[{#1}\right]}   % Expectation
%\newcommand{\E}[1]{\mathrm{E}\!\left[\,{#1}\,\right]}   % Expectation
\newcommand{\E}[1]{\mathbb{E}\!\left[\,{#1}\,\right]}   % Expectation
\newcommand{\EP}[1]{\mathrm{E}_P\!\left[\,{#1}\,\right]}   % Expectation
\newcommand{\Ec}[2]{\mathrm{E}_{#2}\!\left[\,{#1}\,\right]}   % Expectation classical
\newcommand{\iE}[1]{\mathrm{E}[\,{#1}\,]}   % Expectation classical (inline)
\newcommand{\iEP}[1]{\mathrm{E}_P[\,{#1}\,]}   % Expectation classical (inline)
\newcommand{\iEc}[2]{\mathrm{E}_{#2}[\,{#1}\,]}   % Expectation classical
\newcommand{\var}[1]{\mathrm{var}\!\left({#1}\right)}   % Variance
\newcommand{\varc}[2]{\mathrm{var}_{#2}\!\left({#1}\right)}   % Variance classical
\newcommand{\normal}[2]{{\mathcal{N}(#1,#2)}}  % normal distribution
\newcommand{\Poisson}[1]{{\mathrm{Poisson}(#1)}}  % Poisson distribution
\newcommand{\ZIPoisson}[2]{{\mathrm{ZIPoisson}(#1,#2)}}  % zero-inflated Poisson distribution
\newcommand{\Neyman}[2]{{\mathrm{Neyman}(#1,#2)}}  % Neyman Type A distribution
\newcommand{\binomial}[2]{{\mathrm{binomial}(#1,#2)}}  % Neyman Type A distribution
\newcommand{\Beta}[2]{{\mathrm{Beta}(#1,#2)}}  % Beta distribution
\newcommand{\uniform}[2]{{\mathcal{U}(#1,#2)}}  % uniform distribution
\def\RVe{{\mathrm{e}}}
\def\RVv{{\mathrm{v}}}
\def\RVw{{\mathrm{w}}}
\def\RVx{{\mathrm{x}}}
\def\RVxhat{\widehat{\RVx}}
\def\RVX{{\mathrm{X}}}
\def\RVXhat{\widehat{\RVX}}
\def\RVy{{\mathrm{y}}}
\def\RVytilde{{\widetilde{\mathrm{y}}}}
\def\RVyhat{{\widehat{\RVy}}}
\def\RVz{{\mathrm{z}}}
\def\RVa{\upalpha}
\def\RVahat{\widehat{\upalpha}}
\def\RVb{\upbeta}
\def\RVbhat{\widehat{\upbeta}}
\newcommand{\RVxhatL}[1]{\widehat{\RVx}_{#1}}
\def\order{O}
\def\thetaOpt{\theta_{\rm opt}}

\def\flp{f_{\rm lp}}
\def\Flp{F_{\rm lp}}

\def\hd{h^{\rm d}}
\def\Hd{H^{\rm d}}

\def\mun{\mu_{\rm t}}
\def\mut{\mu_{\rm t}}
\def\muw{\mu_{\rm f}}
\def\muf{\mu_{\rm f}}
\def\Deltan{\Delta_{\rm t}}
\def\Deltat{\Delta_{\rm t}}
\def\Deltaw{\Delta_{\rm f}}
\def\Deltaf{\Delta_{\rm f}}
\def\DeltatHat{\widehat{\Delta}_{\rm t}}
\def\DeltawHat{\widehat{\Delta}_{\rm f}}
\def\Nt{N_{\rm t}}
\def\Nw{N_{\rm f}}

% Tables
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}


\def\IndicatorK{\mathbbm{1}_{\{ Y_k > 0\}}}
\def\A{\mathrm{A}}
\def\B{\mathrm{B}}
\def\xmax{x_{\rm max}}

\def\lambdabf{\boldsymbol{\lambda}}
\def\etabf{\boldsymbol{\eta}}
\def\pbf{\mathbf{p}}
\def\vbf{\mathbf{v}}
\def\wbf{\mathbf{w}}
\def\Ybf{\mathbf{Y}}
\def\lambdabfhat{\widehat{\boldsymbol{\lambda}}}
\def\etabfhat{\widehat{\boldsymbol{\eta}}}
\def\lambdahat{\widehat{\lambda}}
\def\etahat{\widehat{\eta}}

\def\utilde{{\widetilde{u}}}
\def\Utilde{{\widetilde{U}}}
\def\MSE{\widehat{\mbox{\footnotesize MSE}}}
\def\MSElower{\mbox{\footnotesize MSE}^-}
\def\MSEupper{\mbox{\footnotesize MSE}^+}
\def\MSEcaption{\widehat{\mbox{\scriptsize MSE}}}
\def\MSElowercaption{\mbox{\scriptsize MSE}^-}
\def\MSEuppercaption{\mbox{\scriptsize MSE}^+}
%\DeclareMathOperator{\Poisson}{Poisson}
\DeclareMathOperator{\Gaussian}{Gaussian}
%\DeclareMathOperator{\binomial}{binomial}
\DeclareMathOperator{\pen}{pen}

\def\MID{\, \| \,}
\newcommand\DKL[2]{D_{\rm KL}( {#1} \MID {#2} )}

\def\CR{Cram{\'e}r--Rao}
\def\etaHat{\widehat{\eta}}
\def\etaML{\widehat{\eta}_{\rm ML}}
\def\etaBaseline{\widehat{\eta}_{\rm baseline}}
\def\etaOracle{\widehat{\eta}_{\rm oracle}}
\def\etaCTQM{\widehat{\eta}_{\rm CTQM}}
\def\etaCTLQM{\widehat{\eta}_{\rm CTLQM}}
\def\etaICA{\widehat{\eta}_{\rm ICA}}
\def\etaTR{\widehat{\eta}_{\rm ICA}}
\def\etaconv{\widehat{\eta}_{\rm conv}}
\def\etaCTML{\widehat{\eta}_{\rm CTML}}
\def\etaDTQM{\widehat{\eta}_{\rm DTQM}}
\def\etaDTLQM{\widehat{\eta}_{\rm DTLQM}}
\def\etaDTML{\widehat{\eta}_{\rm DTML}}
\def\IndicatorK{\mathbbm{1}_{\{ Y_k > 0\}}}
\def\PposMfull{{1 - e^{-\eta}}}
\def\PposM{\rho}
\def\PMD{\mathrm{P}_{\rm MD}}
\def\etaQM{\widehat{\eta}_{\rm QM}}
\def\etaLQM{\widehat{\eta}_{\rm LQM}}
\def\etaML{\widehat{\eta}_{\rm ML}}
\def\etaMLI{\widehat{\eta}_{\rm MLI}}
\def\etaCCMLI{\widehat{\eta}_{\rm CCMLI}}
\def\etaCE{\widehat{\eta}_{\rm CE}}
\def\etaCI{\widehat{\eta}_{\rm CI}}
\def\etaIC{\widehat{\eta}_{\rm IC}}
\def\etaICO{\widehat{\eta}_{\rm ICO}}
\def\etaMtilde{\widehat{\eta}_{\Mtilde}}
\def\etaMax{\eta_{\rm max}}
\def\MBLS{\widehat{M}_{\rm BLS}}
\def\etaconv{\widehat{\eta}_{\rm conv}}
\def\Mtildecorr{\widetilde{M}_{\rm corr}}
\def\um{\si{\micro\meter}}
\def\mm{\si{\milli\meter}}
\def\ms{\si{\milli\second}}
\def\us{\si{\micro\second}}
\def\ns{\si{\nano\second}}
\def\ps{\si{\pico\second}}
\def\pA{\si{\pico\ampere}}
\def\nA{\si{\nano\ampere}}
\def\keV{\si{\kilo\electronvolt}}
\def\eV{\si{\electronvolt}}
\def\V{\si{\volt}}

\def\cmu{{c_{\mu}}}
\def\csig{{c_{\sigma}}}
